COMPS: Conceptual Minimal Pair Sentences for testing Robust Property Knowledge and its Inheritance in Pre-trained Language Models

A characteristic feature of human semantic cognition is its ability to not only store and retrieve the properties of concepts observed through experience, but to also facilitate the inheritance of properties (can breathe) from superordinate concepts (animal) to their subordinates (dog) -- i.e. demonstrate property inheritance. In this paper, we present COMPS, a collection of minimal pair sentences that jointly tests pre-trained language models (PLMs) on their ability to attribute properties to concepts and their ability to demonstrate property inheritance behavior. Analyses of 22 different PLMs on COMPS reveal that they can easily distinguish between concepts on the basis of a property when they are trivially different, but find it relatively difficult when concepts are related on the basis of nuanced knowledge representations. Furthermore, we find that PLMs can demonstrate behavior consistent with property inheritance to a great extent, but fail in the presence of distracting information, which decreases the performance of many models, sometimes even below chance. This lack of robustness in demonstrating simple reasoning raises important questions about PLMs' capacity to make correct inferences even when they appear to possess the prerequisite knowledge.

==> figures/subfigure1.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
    \small
        \begin{quote}
            \textbf{Property:} \textit{can fly}\\
            \textbf{Positive:} \textsc{robin}\\
            \textbf{Negative:} \textsc{penguin}\\
            % \textbf{Negative Concept:} \textsc{penguin}\\
            \textbf{Subordinate:} \textsc{wug}\\
             \textbf{\compsbase{}:} A (\textbf{robin/penguin}) can fly.\\
            \textbf{\compswugs{}:} A wug is a (\textbf{robin/penguin}). Therefore, a wug can fly.
        \end{quote}
        \caption{Instances of \compsbase{} and \compswugs{}.}
        \label{fig:propinheritstim}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.54\textwidth}
        \centering
        \small
        \begin{enumerate}[label=\large\protect\nodeId{\small\arabic*}]
            \item $\log p(\text{can fly.}\mid\text{a robin})$
            \item $\log p(\text{can fly.}\mid\text{a penguin})$
            \item $\log p(\text{can fly.}\mid\text{a wug is a robin. Therefore, a wug})$
            \item $\log p(\text{can fly.}\mid\text{a wug is a penguin. Therefore, a wug})$
        \end{enumerate}
        \caption{Measures considered to analyze property inheritance in \plms, based on the example shown in the figure to the left (\ref{fig:propinheritstim}).}
        \label{fig:propinheritmeasures}
    \end{subfigure}
    \caption{Examples of materials used in our experiments. In this example, \textsc{robin} is the positive concept.}
    \label{fig:propinheritstuff}
    \vspace{-1em}
\end{figure*}

==> figures/subfigure3.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.53\textwidth}
    \small
        \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cl@{}}
\toprule
\textbf{\comps{}} & \textbf{Prefix} \\ \midrule
\textsc{base} & \begin{tabular}[c]{@{}l@{}}$C_{+}$: A robin\\ $C_{-}$: A penguin\end{tabular} \\ \midrule
\textsc{wugs} & \begin{tabular}[c]{@{}l@{}}$C_{+}$: A wug is a robin. Therefore, a wug\\ $C_{-}$: A wug is a penguin. Therefore, a wug\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}c@{}}\textsc{wugs-dist}\\ \footnotesize(\befor)\end{tabular} & \begin{tabular}[c]{@{}l@{}}$C_{+}$: A wug is a robin. A dax is a penguin. Therefore, a wug\\ $C_{-}$:  A wug is a robin. A dax is a penguin. Therefore, a dax\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}c@{}}\textsc{wugs-dist}\\ \footnotesize(\inbetween)\end{tabular} & \begin{tabular}[c]{@{}l@{}}$C_{+}$: A dax is a penguin. A wug is a robin. Therefore, a wug\\ $C_{-}$: A dax is a penguin. A wug is a robin. Therefore, a dax\end{tabular} \\ \bottomrule
\end{tabular}%
}
        \caption{Prefixes used in \comps{}. Here, the property is \textit{can fly}.}
        \label{fig:basewugsstim}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.43\textwidth}
        \centering
         \includegraphics[width=0.9\columnwidth]{figures/distractionparadigm.pdf}
        \caption{Distraction scheme for stimuli in \compswugsdist{}, where the distractor is inserted either \textbf{\textcolor{orang}{before}} or \textbf{\textcolor{purpl}{in between}} each \compswugs{} stimulus.}
        \label{fig:wugsdiststim}
    \end{subfigure}
    \caption{Examples of materials used in our experiments. In this example, \textsc{robin} is the positive concept.}
    \label{fig:compsstim}
    \vspace{-1em}
\end{figure*}

% \begin{table}[]
% \centering

% \caption{}
% \label{tab:stimulitable}
% \end{table}

==> tables/compatibility.tex <==
\def\arraystretch{1.15}
\begin{table}[t!]
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{@{}ccc@{}}
\toprule
\textbf{Hypothesis} & \textbf{Compatibility} & \textbf{Ceiling} \\ \midrule
1 & \textbf{55.6$_{\text{5.6}}$} & \multirow{2}{*}{$\underset{\nodeIdd{1} > \nodeIdd{2}}{\text{67.1}_{\text{4.8}}}$} \\
2 & 11.4$_{\text{1.5}}$ &  \\ \cmidrule(l){2-3}
3 & 13.3$_{\text{2.0}}$ & \multirow{2}{*}{$\underset{\nodeIdd{1} < \nodeIdd{2}}{\text{32.9}_{\text{4.8}}}$} \\
4 & 19.6$_{\text{5.0}}$ &  \\ \bottomrule
\end{tabular}%
}
\caption{Average compatibility scores (and standard deviations) of \plms{} with the four hypotheses regarding the models' property inheritance behavior. Ceiling scores indicate upper-bounds across hypothesis pairs.}
\label{tab:compatibility}
\vspace{-1.6em}
\end{table}

==> tables/comps-results.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccccccccccccccc@{}}
\toprule
 & \textbf{A-b} & \textbf{A-l} & \textbf{A-xl} & \textbf{A-xxl} & \textbf{B-b} & \textbf{B-l} & \textbf{dB-b} & \textbf{dGPT2} & \textbf{dR-b} & \textbf{E-b} & \textbf{E-l} & \textbf{E-s} & \textbf{GPT-J} & \textbf{Neo-1.3b} & \textbf{Neo-125M} & \textbf{Neo-2.7B} & \textbf{GPT2} & \textbf{GPT2-l} & \textbf{GPT2-m} & \textbf{GPT2-xl} & \textbf{GPT} & \textbf{R-b} & \textbf{R-l} \\ \midrule
\textbf{Taxonomic} & \gradient{0.61} & \gradient{0.63} & \gradient{0.63} & \gradient{0.69} & \gradient{0.63} & \gradient{0.64} & \gradient{0.63} & \gradient{0.59} & \gradient{0.60} & \gradient{0.62} & \gradient{0.63} & \gradient{0.61} & \gradient{0.72} & \gradient{0.66} & \gradient{0.56} & \gradient{0.68} & \gradient{0.60} & \gradient{0.67} & \gradient{0.65} & \gradient{0.68} & \gradient{0.66} & \gradient{0.62} & \gradient{0.68} \\
\textbf{Overlap} & \gradient{0.60} & \gradient{0.62} & \gradient{0.62} & \gradient{0.65} & \gradient{0.61} & \gradient{0.61} & \gradient{0.61} & \gradient{0.59} & \gradient{0.61} & \gradient{0.62} & \gradient{0.63} & \gradient{0.60} & \gradient{0.71} & \gradient{0.65} & \gradient{0.60} & \gradient{0.67} & \gradient{0.62} & \gradient{0.66} & \gradient{0.64} & \gradient{0.67} & \gradient{0.65} & \gradient{0.61} & \gradient{0.66} \\
\textbf{Co-oc} & \gradient{0.61} & \gradient{0.63} & \gradient{0.64} & \gradient{0.71} & \gradient{0.63} & \gradient{0.66} & \gradient{0.63} & \gradient{0.57} & \gradient{0.60} & \gradient{0.61} & \gradient{0.63} & \gradient{0.57} & \gradient{0.74} & \gradient{0.66} & \gradient{0.53} & \gradient{0.69} & \gradient{0.61} & \gradient{0.68} & \gradient{0.66} & \gradient{0.71} & \gradient{0.66} & \gradient{0.62} & \gradient{0.68} \\
\textbf{Random} & \gradient{0.77} & \gradient{0.81} & \gradient{0.83} & \gradient{0.87} & \gradient{0.79} & \gradient{0.81} & \gradient{0.82} & \gradient{0.75} & \gradient{0.78} & \gradient{0.79} & \gradient{0.82} & \gradient{0.76} & \gradient{0.90} & \gradient{0.86} & \gradient{0.71} & \gradient{0.87} & \gradient{0.81} & \gradient{0.88} & \gradient{0.86} & \gradient{0.89} & \gradient{0.82} & \gradient{0.80} & \gradient{0.87} \\
\textbf{Overall} & \gradient{0.37} & \gradient{0.40} & \gradient{0.41} & \gradient{0.48} & \gradient{0.40} & \gradient{0.41} & \gradient{0.40} & \gradient{0.36} & \gradient{0.38} & \gradient{0.39} & \gradient{0.41} & \gradient{0.36} & \gradient{0.56} & \gradient{0.47} & \gradient{0.34} & \gradient{0.50} & \gradient{0.39} & \gradient{0.47} & \gradient{0.45} & \gradient{0.50} & \gradient{0.44} & \gradient{0.39} & \gradient{0.46} \\ \bottomrule
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table*}

==> tables/confusion.tex <==
% 1 & \textbf{55.6$_{\text{5.6}}$} & \multirow{2}{*}{$\underset{\nodeIdd{1} > \nodeIdd{2}}{\text{67.1}_{\text{4.8}}}$} \\
% 2 & 11.4$_{\text{1.5}}$ &  \\ \cmidrule(l){2-3}
% 3 & 13.3$_{\text{2.0}}$ & \multirow{2}{*}{$\underset{\nodeIdd{1} < \nodeIdd{2}}{\text{32.9}_{\text{4.8}}}$} \\
% 4 & 19.6$_{\text{5.0}}$ &  \\ \bottomrule

\setcellgapes{5pt}
\makegapedcells
\begin{table}[h]
    \centering
    \resizebox{0.6\columnwidth}{!}{%
    \begin{tabular}{cc|cc}
\multicolumn{2}{c}{}
            &   \multicolumn{2}{c}{\textsc{wugs}} \\
    &       &   \cmark{} &   \xmark{}              \\ 
    \cline{2-4}
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{base}}}
    & \cmark{}   & 55.6$_{\text{5.6}}$   & 11.4$_{\text{1.5}}$                \\
    & \xmark{}   &  13.3$_{\text{2.0}}$   & 19.6$_{\text{5.0}}$                \\ 
    \cline{2-4}
    \end{tabular}}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


==> tables/overall2.tex <==
\begin{table}[]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{\textsc{comps}} & \textbf{$\mathcal{A}$} & $\mathcal{A}^\prime$ \\ \midrule
\textsc{base} & $\text{68.4}_{\text{4.1}}$ & - \\
\textsc{base}$_{\textit{(animal kingdom only)}}$ & $\text{67.1}_{\text{4.8}}$ & - \\
\textsc{wugs} & $\text{68.9}_{\text{5.5}}$ & $\text{55.6}_{\text{5.6}}$ \\
\textsc{wugs-dist}$_{\textit{(\befor)}}$ & $\text{59.2}_{\text{9.5}}$ & $\text{41.3}_{\text{8.8}}$ \\
\textsc{wugs-dist}$_{\textit{(\inbetween)}}$ & $\text{47.2}_{\text{4.5}}$ & $\text{32.8}_{\text{6.8}}$ \\ \bottomrule
\end{tabular}%
}
\caption{Average accuracy (and standard deviation) of models (\textit{N}=22) on each of our \textsc{comps} subsets.}
\label{tab:overall2}
\end{table}

==> tables/overall3.tex <==
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}clrr@{}}
\toprule
\textbf{\textsc{base}} & \textbf{Prop. Inherit.} & \textbf{Acc.} & \textbf{Rel. Acc.} \\ \midrule
\multirow{3}{*}{$\text{67.1}_{\text{4.8}}$} & \compswugs{} & $\text{55.6}_{\text{5.6}}$ & $\text{82.8}_{\text{2.8}}$ \\
 & \textsc{comps-wugs-dist}$_{\text{\befor}}$ & $\text{41.3}_{\text{8.8}}$ & $\text{61.1}_{\text{8.9}}$ \\
 & \textsc{comps-wugs-dist}$_{\text{\inbetween}}$ & $\text{32.8}_{\text{6.8}}$ & $\text{49.5}_{\text{11.6}}$ \\ \bottomrule
\end{tabular}%
}
\caption{Average Performance (accuracy and standard deviation) of models (\textit{N} = 22) on each of our \textsc{comps} subsets. Chance performance is 50\%.}
\label{tab:overall3}
\end{table}
